Drinfeld center of planar algebra

We introduce fusion, contragradient and braiding of Hilbert affine representations of a subfactor planar algebra $P$ (not necessarily having finite depth). We prove that if $N \subset M$ is a subfactor realization of $P$, then the Drinfeld center of the $N$-$N$-bimodule category generated by $_N L^2 (M)_M$, is equivalent to the category of Hilbert affine representations of $P$ satisfying certain finiteness criterion. As a consequence, we prove Kevin Walker's conjecture for planar algebras.

==> texfiles/affmod.tex <==
\section{Analysis  of affine modules}
In this section,
%we will first analyze the space of affine morphisms and prove some of their basic properties which will be very useful in the later sections.
%Throughout this section, $P$ will denote a (spherical) subfactor planar algebra.
%Using this,
we will lay down a method of determining a large class of affine $P$-modules for a subfactor planar algebra (possibly having infinite depth).
%The analysis of affine morphisms will also show that they are intimately linked with the commutativity constraints appearing in Drinfeld's center construction.
Some of the materials in this section are motivated by our treatment of affine modules with zero weight in {\bf Pending Section 4}, which we will avoid mentioning at every step.

For $\vlon k \in \t{Col}$, consider the $*$-affine $P$-module $H^{\vlon k}$ defined by:

\noindent {\em Inner product spaces:}
$H^{\vlon k}_{\eta l}$ is the vectors space $AP_{\vlon k, \eta l}$ with inner product given by $\lab \cdot , \cdot \rab_{\vlon k}$.

\noindent {\em Action of affine morphisms:}
Action of $a \in AP_{\eta l, \gamma m}$ is given by $ H^{\vlon k}_{\eta l} \ni b \os{H^{\vlon k}_a}{\longmapsto} a\circ b \in H^{\vlon k}_{\gamma m}$.
\begin{prop}\label{bounded}
$H^{\vlon k}$ is a bounded.
\end{prop}
\begin{proof}
Fix $a \in AP_{\eta l, \gamma m}$.
There exists $s \in \N_0$ and $x \in P_{\gamma (l+m+s)}$ such that $a = \psi^s_{\eta l, \gamma m} (x)$.
Now, for all $b = \psi^t_{\vlon k, \eta l} (y)$, we have
\[
\norm{H^{\vlon k}_a (b)}^2_{\vlon k} = \omega_{\vlon k} (b^* \circ a^* \circ a \circ b) = \delta^{-(2k+s+t)} \us{\alpha}{\sum} P_{
\psfrag{u*}{$u^*_\alpha$}
\psfrag{u}{$u_\alpha$}
\psfrag{2m}{$2m$}
\psfrag{2l}{$2l$}
\psfrag{2k}{$2k$}
\psfrag{t}{$t$}
\psfrag{s}{$s$}
\psfrag{y*}{$y^*$}
\psfrag{y}{$y$}
\psfrag{x}{$x$}
\psfrag{x*}{$x^*$}
\includegraphics[scale=0.15]{figures/affmod/abnorm.eps}
} = f(w)
\]
where $f := \delta^{-(2k+s+t)} \us{\alpha}{\sum} P_{
\psfrag{u*}{$u^*_\alpha$}
\psfrag{u}{$u_\alpha$}
\psfrag{2s}{$2s$}
\psfrag{2l}{$2l$}
\psfrag{2k}{$2k$}
\psfrag{t}{$t$}
\psfrag{s}{$s$}
\psfrag{y*}{$y^*$}
\psfrag{y}{$y$}
\psfrag{g}{$\gamma$}
\includegraphics[scale=0.15]{figures/affmod/f.eps}
} : P_{\gamma 2(l+s)} \ra \C$, $w := P_{
\psfrag{2m}{$2m$}
\psfrag{2l+2s}{$2(l+s)$}
\psfrag{g}{$\gamma$}
\psfrag{x}{$x$}
\psfrag{x*}{$x^*$}
\includegraphics[scale=0.15]{figures/affmod/w.eps}
}$ and $\{ u_\alpha \}_\alpha$ is an orthonormal basis of $P_{\vlon (s+t)}$.
Note that $f$ is a positive functional on $P_{\gamma 2(l+s)}$ since for all $0 \leq v \in P_{\gamma 2(l+s)}$, we may write $f(v) = \norm{\psi^s_{\eta l, \gamma (l+s)} (v^{1/2}) \circ \psi^t_{\vlon k, \eta l} (y)}^2_{\vlon k} >0 $.
Clearly, $w \geq 0$; so, $\norm{H^{\vlon k}_a (b)}^2_{\vlon k} \leq \norm{w} f(1_{P_{\gamma 2(l+s)}})$ where $w$ gets the $C^*$-norm from $P_{\gamma 2(l+s)}$.
In order to compute $f(1_{P_{\gamma 2(l+s)}})$, we consider an orthonormal basis $\{ v_\beta \}_\beta$ of $P_{\vlon t}$.
Observe that (a) $\{ \tilde v_\beta := P_{RI^s_{\vlon t}} (v_\beta) \}_\beta$ is an orthonormal subset of $P_{\vlon (s+t)}$ and (b) $P_{RE^s_{\vlon (s+t)}} (v) = 0$ whenever $v \in \{ \tilde v_\beta \}^\perp_\beta$.
Without loss of generality, we may assume $\{ \tilde v_\beta \}_\beta \subset \{ u_\alpha \}_\alpha$.
Using (a) and (b), we may conclude $f( 1_{P_{\gamma (l+s)}} ) = \delta^s \norm{b}^2_{\vlon k}$. This ends the proof.
\end{proof}
\begin{cor}\label{findepregmod}
If the depth of $P$ is finite ($d$ say), then any irreducible Hilbert affine $P$-module is isomorphic to a submodule of $H^{+ k}$ for all $k > d /2$.
\end{cor}
\begin{proof}
{\bf Pending}
\end{proof}
Note that Corollary \ref{findepregmod} fails in the infinite depth case.
By Proposition \ref{bounded}, we may consider the Hilbert affine $P$-module $\mcal H^{\vlon k}$ where $\mcal H^{\vlon k}_{\eta l}$ is the completion of the inner product space $H^{\vlon k}_{\eta l}$ and  $\mcal H^{\vlon k}$-action of an affine morphisms is the unique extension of the $H^{\vlon k}$-action.
Now, $H^{\vlon k}_{\eta l}$'s have a right $AP_{\vlon k,\vlon k}$-action, denoted by $\rho^{\vlon k}_{\eta l} : AP_{\vlon k, \vlon k} \ra \t{End}_\C (H^{\vlon k}_{\eta l})$, which commutes with the $H^{\vlon k}$-action of affine morphisms on the left.
\begin{cor}
For all $\vlon k, \eta l \in \t{Col}$ and $a \in AP_{\vlon k, \vlon k}$, $\rho^{\vlon k}_{\eta l} (a)$ is bounded.
\end{cor}
\begin{proof}
Using spherical isotopy, we may write $\delta^{2k} \omega_{\vlon k} (b_1 \circ b_2) = \delta^{2l} \omega_{\eta l} (b_2 \circ b_1)$ for all $b_1 \in AP_{\eta l , \vlon k}$ and $b_2 \in AP_{\vlon k , \eta l}$.
If $b \in H^{\vlon k}_{\eta l} = AP_{\vlon k , \eta l}$, then applying this relation and Proposition \ref{bounded}, we get
\[
\norm{\rho^{\vlon k}_{\eta l} (a) (b) }^2_{\vlon k} = \omega_{\vlon k} (a^* \circ b^* \circ b \circ a) = \delta^{2(l-k)} \norm{H^{\eta l}_{a^*} (b^*) }^2_{\eta l} \leq \delta^{2(l-k)} \norm{H^{\eta l}_{a^*} }^2 \norm{b^*}^2_{\eta l} = \norm{H^{\eta l}_{a^*} }^2 \norm{b}^2_{\vlon k}.
\]
\end{proof}
We may extend $\rho^{\vlon k}_{\eta l}$ to a right action of $AP_{\vlon k, \vlon k}$ on $\mcal H^{\vlon k}_{\eta l}$, which we denote by the same symbol $\rho^{\vlon k}_{\eta l} : AP_{\vlon k , \vlon k} \ra \mcal B ( \mcal H^{\vlon k}_{\eta l} )$.
Set $L^{\vlon k} := (\mcal H^{\vlon k}_{AP_{\vlon k , \vlon k}} )'' \subset \mcal B (\mcal H^{\vlon k}_{\vlon k})$ which is a finite von Neumann algebra with a faithful normal tracial state given by $\tau_{\vlon k} := \lab \hat 1_{AP_{\vlon k, \vlon k}} , \cdot (\hat 1_{AP_{\vlon k, \vlon k}} ) \rab_{\vlon k} : L^{\vlon k} \ra \C$.
Note that $\tau_{\vlon k} (\mcal H^{\vlon k}_a) = \omega_{\vlon k} (a)$ for all $a \in AP_{\vlon k, \vlon k}$.
\begin{lem}\label{ract}
The anti-algebra $*$-homomorphism $\rho^{\vlon k}_{\eta l} : AP_{\vlon k , \vlon k} \ra \mcal B ( \mcal H^{\vlon k}_{\eta l} )$ extends to a normal anti-algebra $*$-homomorphism from $L^{\vlon k}$ to $\mcal B (\mcal H^{\vlon k}_{\eta l})$ for all $\eta l \in \t{Col}$.
\end{lem}
\begin{proof}
The case $k=0$ is already shown in {\bf Pending}; so, without loss of generality, we may assume $k \neq 0$.
In the remaining, we will frequently use the identity \begin{equation}\label{hrcomm}
\mcal H^{\vlon k}_{a} \circ\mcal \rho^{\vlon k}_{\eta l} (b) = \rho^{\vlon k}_{\nu m} (b) \circ \mcal H^{\vlon k}_{a} \t{ for all } a \in AP_{\eta l , \nu m}, b \in AP_{\vlon k, \vlon k}.
\end{equation}
Set $W_{\eta l} := (\rho^{\vlon k}_{\eta l} (AP_{\vlon k, \vlon k}))'' \subset \mcal B( \mcal H^{\vlon k}_{\eta l})$.
Note that we have an anti-algebra $*$-isomorphism $L^{\vlon k} \ni \mcal H^{\vlon k}_a \mapsto J (\mcal H^{\vlon k}_a )^* J = \rho^{\vlon k}_{\vlon k} (a) \in W_{\vlon k}$ for $a \in AP_{\vlon k,\vlon k}$ where $J$ is the canonical conjugate linear unitary on $L^2(L^{\vlon k} , \tau_{\vlon k}) \cong \mcal H^{\vlon k}_{\vlon k}$.
So, it is enough to show  that $W_{\vlon k} \ni \rho^{\vlon k}_{\vlon k} (a) \os{\alpha_{\eta l}}{\longmapsto} \rho^{\vlon k}_{\eta l} (a) \in W_{\eta l}$ for $a \in AP_{\vlon k, \vlon k}$, extends to a normal $*$-homomorphism.
%%%%%%%%%%%%%%%%%%%%
\comments{
There is nothing to prove when $\eta l = \vlon k$.
If $\eta l = -\vlon k$, then consider the unitary $\mcal H^{\vlon k}_r : \mcal H^{\vlon k}_{\vlon k} \ra \mcal H^{\vlon k}_{-\vlon k}$ given by the action of the `rotation' morphism $r := AR_{\vlon k} \in AP_{\vlon k, -\vlon k}$ (as defined in Figure {\bf Pending}).
By the intertwing property $\mcal H^{\vlon k}_r \circ \rho^{\vlon k}_{\vlon k} (\cdot ) \circ \mcal H^{\vlon k}_{r^*} = \rho^{\vlon k}_{-\vlon k} (\cdot )$, we get the required result.
}%%%%%%%%%%%%%%%%%%%%

Before proceeding further, we set up some notations.
Let $c_{\kappa m, \nu n}$ denote the element  $\psi^0_{\kappa m, \nu n} (1_{P_{\nu (m+n)}})$ or  $\psi^1_{\kappa m, \nu n} (1_{P_{\nu (m+n+1) } })$ in $AP_{\kappa m, \nu n}$ according as $\kappa = \nu$ or $\kappa \neq\nu$.
It is routine to verify $c^*_{\kappa m, \nu n} \circ c_{\kappa m, \nu n} = \delta^{n-m} 1_{AP_{\kappa m, \kappa m}}$ whenever $n \geq m$.

Set $U := \delta ^{(k-l)/2} \mcal H^{\vlon k}_{c_{\vlon k, \eta l}} : \mcal H^{\vlon k}_{\vlon k} \ra \mcal H^{\vlon k}_{\eta l}$ (resp., $\delta ^{(l-k)/2} \mcal H^{\vlon k}_{c_{\eta l, \vlon k}} : \mcal H^{\vlon k}_{\eta l} \ra \mcal H^{\vlon k}_{\vlon k}$) when $l > k$ (resp., $k \geq l$).
Note that $U$ is an isometry; this along with identity \ref{hrcomm} implies $p := UU^* \in \mscr P ( W'_{\eta l} )$ (resp., $\mscr P ( W'_{\vlon k} )$).
Thus, we get a normal $*$-homomorphism $W_{\eta l} \ni x \os{\alpha}{\mapsto} U^* x U \in \mcal B (\mcal H^{\vlon k}_{\vlon k})$ (resp., $W_{\vlon k} \ni x \os{\alpha}{\mapsto} U^* x U \in \mcal B (\mcal H^{\vlon k}_{\eta l})$); so, its range is a von Neumann algebra.
Again, using identity \ref{hrcomm}, $\alpha \left( \rho^{\vlon k}_{\eta l} (a) \right) = \rho^{\vlon k}_{\vlon k} (a)$ (resp., $\alpha \left( \rho^{\vlon k}_{\vlon k} (a) \right) = \rho^{\vlon k}_{\eta l} (a)$) for all $a \in AP_{\vlon k,\vlon k}$ which gives $\t{Range }\alpha = W_{\vlon k}$ (resp., $W_{\vlon k}$).
This proves the required result for $k \geq l$.


To complete the proof for $l > k$, it will be enough to show $\alpha$ is injective.
Note that the central support of $p$ is $1$ in $W_{\eta l}$ since $\mcal H^{\vlon k}_{ AP_{\eta l, \eta l} } (p ( c_{\eta l}) ) = H^{\vlon k}_{\eta l}$ (where $c_{\eta l}$ is treated as an element of $\mcal H^{\vlon k}_{\eta l}$) and $\mcal H^{\vlon k}_{AP_{\eta l, \eta l}} \subset W'_{\eta l}$ (by identity \ref{hrcomm}).
Thus, $W_{\eta l} \ni x \mapsto xp \in W_{\eta l} p$ is an isomorphism.
This makes $W_{\eta l} \ni x \os{\alpha}{\mapsto} U^* x U \in W_{\vlon k}$ injective, and hence, an isomorphism too.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\comments{
\noindent {\bf Case 1:}
Suppose $l > k$.
Let $c_{\eta l}$ denote the element 
%\delta ^{(k-l)/2} \psi^{1 - \delta_{\eta=-1}}_{\vlon k, \vlon l} (1_{P_{\eta (k+l)}})
$\psi^0_{\vlon k, \eta l} (1_{P_{\eta (k+l)}})$ or  $\delta ^{(k-l)/2} \psi^1_{\vlon k, \eta l} (1_{P_{\eta (k+l)) } })$ in $AP_{\vlon k,\eta l}$ according as $\eta$ is $\vlon$ or $-\vlon$; set $U := \delta ^{(k-l)/2} \mcal H^{\vlon k}_{c_{\eta l}} : \mcal H^{\vlon k}_{\vlon k} \ra \mcal H^{\vlon k}_{\eta l}$ and $p:= UU^* = \delta ^{k-l} \mcal H^{\vlon k}_{ c_{\eta l} \circ c^*_{\eta l} }$.
Note that $U$ is an isometry; this along with identity \ref{hrcomm} implies $p \in \mscr P ( W'_{\eta l} )$.
Moreover, the central support of $p$ is $1$ in $W_{\eta l}$ since $\mcal H^{\vlon k}_{ AP_{\eta l, \eta l} } (p ( c_{\eta l}) ) = H^{\vlon k}_{\eta l}$ (where $c_{\eta l}$ is treated as an element of $\mcal H^{\vlon k}_{\eta l}$) and $\mcal H^{\vlon k}_{AP_{\eta l, \eta l}} \subset W'_{\eta l}$ (by identity \ref{hrcomm}).
Thus, $W_{\eta l} \ni x \mapsto xp \in W_{\eta l} p$ is an isomorphism and thereby, we get a injective $*$-algebra homomorphism $W_{\eta l} \ni x \os{\alpha}{\mapsto} U^* x U \in \mcal B (\mcal H^{\vlon k}_{\vlon k})$.
Since $\alpha$ is normal, therefore its range is a von Neumann algebra.
On the other hand, $\alpha \left( \rho^{\vlon k}_{\eta l} (a) \right) = \rho^{\vlon k}_{\vlon k} (a)$ for all $a \in AP_{\vlon k,\vlon k}$ which gives $\t{Range }\alpha = W_{\vlon k}$.
Hence, $\alpha_{\eta l}$ is given by $\alpha^{-1}$.

\noindent {\bf Case 2:} Suppose $l < k$.
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{proof}
\begin{lem}\label{w*lem}
The unital $*$-algebra homomorphism $AP_{\eta l , \eta l} \ni a \mapsto \mcal H^{\vlon k}_a \in \mcal B(\mcal H^{\vlon k}_{\eta l})$ extends to a normal homomorphism from $L^{\eta l}$ to $\mcal B(\mcal H^{\vlon k}_{\eta l})$ for all $\eta l \in \t{Col}$.
\end{lem}
\begin{proof}
Consider the conjugate linear unitary $\mcal H^{\vlon k}_{\eta l} \ni b \os{J}{\mapsto} \delta^{l-k} b^* \in \mcal H^{\eta l}_{\vlon k}$ whose adjoint is given by $\mcal H^{\eta l}_{\vlon k} \ni b \os{J}{\mapsto} \delta^{k-l} b^* \in \mcal H^{\vlon k}_{\eta l}$.
By Lemma \ref{ract}, the map $L^{\eta l} \ni x \mapsto J^* \rho^{\eta l}_{\vlon k} (x^*) J \in B(\mcal H^{\vlon k}_{\eta l})$ is normal; this also sends $\mcal H^{\eta l}_a$ to $\mcal H^{\vlon k}_a$ for all $a \in AP_{\eta l , \eta l}$.
\end{proof}
Lemma \ref{w*lem} gives $\mcal H^{\vlon k}_{\eta l}$ a left $L^{\eta l}$-module structure (in fact, a $L^{\eta l}$-$L^{\vlon k}$-bimodule structure).
This prompts us to introduce the following definition where  the $C^*$-algebra completion of $AP_{\vlon k , \vlon k}$ with respect to its action on $\mcal H^{\vlon k}_{\vlon k}$ is denoted by $C^{\vlon k}$ ($\subset L^{\vlon k}$ as a $C^*$-subalgebra).
\begin{defn}
A Hilbert affine $P$-module $V$ is said to be {\em $C^*$-affine $P$-module} (resp., {\em $W^*$-affine $P$-module}) if the $V$-action of $AP_{\eta l, \eta l}$ on $V_{\eta l}$, extends to an action of the $C^*$-algebra $C^{\eta l}$ (resp., von Neumann algebra $L^{\eta l}$) for all $\eta l \in \t{Col}$.
\end{defn}
By Lemma \ref{w*lem}, $\mcal H^{\vlon k}$'s are all $W^*$- (and hence, $C^*$-) affine $P$-modules.
This brings us to the main theorem of this section which characterizes all $C^*$- and $W^*$-affine $P$-module.
\begin{thm}
For every left $C^{\vlon k}$-module (resp., $L^{\vlon k}$-module) $\mcal K$, there exists unique $C^*$- (resp., $W^*$-) affine $P$-module, say $\lab \mcal K \rab$, such that $\mcal K$ and $\lab \mcal K \rab_{\vlon k}$ are isometrically isomorphic as $AP_{\vlon k, \vlon k}$-modules, and $\left[ \lab \mcal K \rab_{\vlon k} \right] = \lab \mcal K \rab$.
Moreover, every $C^*$- (resp., $W^*$-) affine $P$-module can be expressed as a (possibly infinite) direct sum of modules of these type.
\end{thm}
\begin{proof}
Uniqueness easily follows from Remark \ref{affmodmor}, and thereby, any finitely supported $C^*$- or $W^*$-affine $P$-module is of the above form.
Now, any $C^*$- (resp., $W^*$-) affine $P$-module decomposes into a direct sum of finitely supported $C^*$- (resp., $W^*$-) affine $P$-modules; this gives the last statement. Now, it remains to construct $\lab \mcal K \rab$; we will first work in the $C^*$-setting.
For $\eta l \in \t{Col}$, consider the vector space $\widetilde {\mcal K}_{\eta l} := AP_{\vlon k , \eta l} \otimes \mcal K$ and the following sesquilinear form on it
\[
\widetilde {\mcal K}_{\eta l} \times \widetilde {\mcal K}_{\eta l} \ni (a \otimes \xi , b \otimes \zeta) \os{\lab \cdot , \cdot \rab} \longmapsto \lab \xi , (a^* \circ b) \zeta \rab_{\mcal K} \in \C
\]
where we identify elements of $AP_{\vlon k, \vlon k}$ with those of $C^{\vlon k}$ via the inclusion map.
Let $x = \us{i \in I} \sum a_i \otimes \xi_i \in \widetilde {\mcal K}_{\eta l}$ for a finite indexing set $I$.
If $s = \us{i,j} \sum \left[ E_{i,j} \otimes (a^*_i \circ a_j) \right] \in M_I \otimes A_{\vlon k , \vlon k} \subset M_I \otimes C^{\vlon k} \hookrightarrow \mcal B ( l^2 (I) \otimes \mcal H^{\vlon k}_{\vlon k})$ and $\tilde \xi = \us{i \in I} \sum e_i \otimes \xi_i \in l^2 (I) \otimes \mcal K$, then $\lab x , x \rab = \lab \tilde \xi , s( \tilde \xi )\rab_{ l^2 (I) \otimes \mcal K}$.
Now, for any $\tilde \zeta = \us{i \in I} \sum e_i \otimes \zeta_i \in l^2 (I) \otimes \mcal H^{\vlon k}_{\vlon k}$, we calculate $\lab \tilde \zeta , s(\tilde \zeta ) \rab_{ l^2 (I) \otimes \mcal H^{\vlon k}_{\vlon k} } = \norm{\us{i \in I} \sum \mcal H^{\vlon k}_{a_i} (\zeta_i) }^2_{ \mcal H^{\vlon k}_{\eta l} } \geq 0$; so, $s$ is a positive element of the $C^*$-algebra $M_I \otimes C^{\vlon k}$.
Then, by complete positivity of representations of $C^*$-algebras, we get $\lab x , x \rab \geq 0$.
Thus, the above form is non-negative definite.
Set $\lab \mcal K \rab_{\eta l}$ as the Hilbert space completion of the quotient of $\widetilde {\mcal K}_{\eta l}$ over the null space of the form.

We will next define the action of affine morphisms. Fix $b \in AP_{\eta l , \nu m}$ and let $x$, $s$ and $\tilde \xi$ be as above.
%$x  = \us{i \in I} \sum a_i \otimes \xi_i \in \widetilde {\mcal K}_{\eta l}$.
Set $y  = \us{i \in I} \sum (b \circ a_i) \otimes \xi_i \in \widetilde {\mcal K}_{\nu m}$ and $t = \us{i,j} \sum \left[ E_{i,j} \otimes (a^*_i \circ b^* \circ b \circ a_j) \right]$.
%and $s = \us{i,j} \sum \left[ E_{i,j} \otimes (a^*_i \circ a_j) \right]$.
Now, using the faithful representation of $M_I \otimes C^{\vlon k}$ on $l^2(I) \otimes \mcal H^{\vlon k}_{\vlon k}$, it is easy to check that $t \leq \norm {\mcal H^{\vlon k}_b}^2 s$.
So, $\lab y , y \rab = \lab \tilde \xi , t( \tilde \xi) \rab_{l^2(I) \otimes \mcal K} \leq \norm {\mcal H^{\vlon k}_b}^2 \lab \tilde \xi , s( \tilde \xi) \rab_{l^2(I) \otimes \mcal K} = \norm {\mcal H^{\vlon k}_b}^2 \lab x , x \rab$.
Thus, $\lab \mcal K \rab_{\eta l} \ni \left[ \us {i \in I} \sum a_i \otimes \xi_i \right] \mapsto  \left[ \us {i \in I} \sum (b \circ a_i) \otimes \xi_i \right] \in \lab \mcal K \rab_{\nu m}$ gives a bounded linear operator which we set as the action of $b$ denoted by  $\lab \mcal K \rab_b$.

Clearly, $\mcal K$ and $\lab  \mcal K \rab_{\vlon k}$ are isometrically isomorphic as $AP_{\vlon k ,\vlon k}$-modules.
Since $\left[ AP_{\vlon k, \eta l} \otimes \mcal K \right]$ is a subset of $\t{span} \left( \lab \mcal K \rab_{ AP_{\vlon k, \eta l} } \left[ AP_{\vlon k, \vlon k} \otimes \mcal K \right]  \right)$, therefore $\left[ \lab \mcal K \rab_{\vlon k} \right] = \lab \mcal K \rab$.
It remains to show that $\lab \mcal K \rab$ is $C^*$ for which it is enough to check $\norm{\lab \mcal K \rab_b} \leq \norm{b}_{ C^{\eta l} }$ for all $b \in AP_{\eta l, \eta l}$, $\eta l \in \t{Col}$.
In the above calculations, we have already found $\norm{\lab \mcal K \rab_b} \leq \norm{\mcal H^{\vlon k}_b}$; the rest follows from the fact that the action of $AP_{\eta l , \eta l}$ on $\mcal H^{\vlon k}_{\eta l}$ extends to an action of the von Neumann algebra $L^{\eta l}$ and hence, of the $C^*$-algebra $C^{\eta l}$.

In the $W^*$ setting, we may carry out the same operation as in the $C^*$ case; however, we end up getting:

(i) $\lab \mcal K \rab_{\eta l} := \mcal H^{\vlon k}_{\eta l} \boxtimes \mcal K$ where $\btimes$ denotes Connes-fusion over $L^{\vlon k}$ with respect to the trace $\tau_{\vlon k}$ and

(ii) $\lab \mcal K \rab_a := \mcal H^{\vlon k}_a \btimes \t{id}_{\mcal K} : \lab \mcal K \rab_{\eta l} \ra \lab \mcal K \rab_{\nu m}$ for $a \in AP_{\eta l , \nu m}$.

By construction, $\lab \mcal K \rab$ satisfies the $W^*$-property.
This ends the proof.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\comments{
\begin{defn}
A Hilbert affine $P$-module $V$ is said to be {\em $W^*$-affine $P$-module} if the $V$-action of $AP_{\eta l, \eta l}$ on $V_{\eta l}$, extends to an action of the von Neumann algebra $L^{\eta l}$. 
\end{defn}
By Lemma \ref{w*lem}, $\mcal H^{\vlon k}$'s are all $W^*$-affine $P$-modules.
This brings us to the main theorem of this section which characterizes all $W^*$-affine $P$-module.
\begin{thm}
For every left $L^{\vlon k}$-module $\mcal K$, there exists unique $W^*$-affine $P$-module, say $\lab \mcal K \rab$, such that $\mcal K$ and $lab \mcal K \rab_{\vlon k}$ are isometrically isomorphic as $AP_{\vlon k, \vlon k}$-modules, and $\left[ \lab \mcal K \rab_{\vlon k} \right] = \lab \mcal K \rab$. Moreover, every $W^*$-affine $P$-module 
can be expressed as a (possibly infinite) direct sum of modules of these type.
\end{thm}
\begin{proof}
Uniqueness easily follows from Remark \ref{affmodmor}, and thereby, any finitely supported $W^*$-affine $P$-module is of the above form.
Now, any $W^*$-affine $P$-module decomposes into a direct sum of finitely supported $W^*$-affine $P$-modules; this gives the last statement. Now, it remains to construct $\lab \mcal K \rab$.
For $\eta l, \nu m \in \t{Col}$, $a \in AP_{\vlon k, \eta l}$, define

(i) $\lab \mcal K \rab_{\eta l} := \mcal H^{\vlon k}_{\eta l} \boxtimes \mcal K$ where $\btimes$ denotes Connes-fusion over $L^{\vlon k}$ with respect to the trace $\tau_{\vlon k}$ and

(ii) $\lab \mcal K \rab_a := \mcal H^{\vlon k}_a \btimes \t{id}_{\mcal K} : \lab \mcal K \rab_{\eta l} \ra \lab \mcal K \rab_{\nu m}$.

Clearly, $\mcal K$ and $\lab  \mcal K \rab_{\vlon k} = \mcal H^{\vlon k}_{\vlon k} \btimes \mcal K$ are isometrically isomorphic as $L^{\vlon k}$-modules.
Since $( AP_{\vlon k , \eta l} ) \hat{}$ is a dense subset of bounded vectors in $\mcal H^{\vlon k}_{\vlon k}$, we may conclude $\lab \mcal K \rab$ is generated by $\lab \mcal K \rab_{\vlon k}$.
By construction, $\lab \mcal K \rab$ satisfies the $W^*$-property.
This ends the proof.
\end{proof}
}%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{rem}
The above process of extension to a Hilbert affine $P$-module might fail if one starts with a Hilbert space representation of $AP_{\vlon ,\vlon k}$ instead of the $C^*$-algebra $C^{\vlon k}$.
However, any Hilbert affine $P$-module $V$ with finite support can be re-constructed in this way from $V_{\vlon k}$ with $k$ exceeding the support of $V$.
\end{rem}
We will work out some example in the latter sections where such extension works and also some counter examples where it does not.
